Execution of Partial State Machine Models

The iterative and incremental nature of software development using models typically makes a model of a system incomplete (i.e., partial) until a more advanced and complete stage of development is reached. Existing model execution approaches (interpretation of models or code generation) do not support the execution of partial models. Supporting the execution of partial models at the early stages of software development allows early detection of defects, which can be fixed more easily and at a lower cost. This paper proposes a conceptual framework for the execution of partial models, which consists of three steps: static analysis, automatic refinement, and input-driven execution. First, a static analysis that respects the execution semantics of models is applied to detect problematic elements of models that cause problems for the execution. Second, using model transformation techniques, the models are refined automatically, mainly by adding decision points where missing information can be supplied. Third, refined models are executed, and when the execution reaches the decision points, it uses inputs obtained either interactively or by a script that captures how to deal with partial elements. We created an execution engine called PMExec for the execution of partial models of UML-RT (i.e., a modeling language for the development of soft real-time systems) that embodies our proposed framework. We evaluated PMExec based on several use-cases that show that the static analysis, refinement, and application of user input can be carried out with reasonable performance and that the overhead of approach, which is mostly due to the refinement and the increase in model complexity it causes, is manageable. We also discuss the properties of the refinement formally and show how the refinement preserves the original behaviors of the model.

==> sections/8-acknowledgments.tex <==
\section*{Acknowledgment}

This work is supported by the Natural Science and Engineering Research Council of Canada, the Ontario Ministry of Research and Innovation, Ericsson Canada, and EfficiOS.

\pagebreak

==> sections/RunningExample.tex <==
\section{ILLUSTRATIVE Example}






%Inspired by paper \cite{HAREL1Statechart}, 
We use a simplified digital watch as an illustrative example to explain our formalization, different types of partiality, and show how our approach works. A full description of digital watch are discussed by Harel \cite{HAREL1Statechart}.   
The watch provides the simple functionalities including showing time and display light (on/off).  As shown in Figure \ref{fig:digiwatch}, the watch consists of \textit{CoreWatch} and \textit{Display} processes. Figure \ref{fig:messages} list the input and output messages by the both processes. The \textit{Display} supports displaying time in normal and light modes. The \textit{CoreWatch} is responsible for tracking current time and updating it in the \textit{Display} by sending a $setT$ message. Also, it  allows users to turn on \& off of the \textit{Display} light by pressing a button ($BA$). We assume that another process which is not discussed here, manages reading the button and sends the related message ($BA$) to the \textit{watchCore}. $tout_1$ and $tout_2$ are timing messages which are produced by another process which is part of the \textit{RTS} and its detail is not discussed here.   

The behaviour model of $Display$ is shown in Figure \ref{fig:display} where each transition and state is given a name and 5-tuple of each transition is specified. \textit{Display} process starts by taking  transitions $t1$ and $t2$ (initial states) sequentially and goes to the $normal$ state. It then stays in $normal$ state until a new message is received. If a $trigL$ message is received, it takes the transition $t3$ and goes the $light$ state in which if a $trigL$ message is received, it goes back to the $normal$ state by taking the transition $t4$. Transitions $t5$, $t6$ are group transitions (i.e., a transition started from a composite state) which are connected to the history state ($H$) state. A group transition is taken for all basic states inside the related composite state.  
This implies that transition $t5$ is executed in $normal$ and $light$ states when message $setD$ is received and returns to the same state after execution since its target is a history state. Similarly, transition $t6$ is executed when a message $ack$ is received.  


The behaviour model of \textit{CoreWatch} is shown in Figure \ref{fig:watchcore}. \textit{CoreWatch} process starts by taking transitions $t1$ and goes to the $checking$ state. In $checking$ state it executes the transition $t2$ when $tou_1$ message is received that is a timing message sent by \textit{RTS} every 5 seconds. In $checking$ state if a message $ack$ is received, it takes transition $t3$ and goes to $working states$ in which it executes the $t4$, $t5$ when messages  $tout_2$ and $BA$ are received. $tou_2$ is a timing message which is sent by $RTS$ every one second, and $BA$ is received when the button $BA$ is pressed. Transitions such as $t2,t4,t5$ with identical source and target are called self transition (i.e.,a given transition $t$ such that $src(t)=tar(t)$).  

\noindent
\textbf{Examples of Helper Functions.} 
Let call the \textit{Display} state machine $dsm$. $sts(dsm)$ returns $\{in1, on, en1\}$, while $\alpha sts(dsm)$ returns $\{in1, en1$ $on,$ $H, in2, normal, light\}$. $trs(dms)$ returns $\{t1,t5,t6\}$ while $\{t1,t5,t6$ $t2,t3,t4\}$. $adj(in1 \in sts(dsm))$ returns $\{on\}$ and  $adj(in2 \in sts(dsm))$ returns $\{on, H, normal, light\}$. $kind(in1 \in sts(dsm))$ and $kind (en1 \in sts(dsm))$ return $\{P\}$, $kind(on \in sts(dsm))$ returns $C$, and $kind(on \in sts(on))$ returns $N$. $typ(t1 \in trs(dms))$ returns $P2x$ and $typ(t3 \in trs(dms))$ and $typ(t5 \in trs(dms))$ return $N2x$. $par(normal \in sts(on))$ returns $on$, and $\alpha par(normal \in sts(on))$ returns $\{on,dsm\}$. 
$lvl(normal \in sts(on))$ returns $2$, and $\alpha par(on \in sts(dsm))$ returns $1$. $\alpha stp(dsm)$ returns $\{\langle t1,t2 \rangle\, \langle t3 \rangle, \langle t4 \rangle, \langle t5 \rangle\, \langle t6 \rangle\ \}$

%it updates the time by sending related messages to $display$ by executing of  the transition $t6$ every one second. If the button $A$ is pressed, it executes the transition $t5$  and reaches the $stopWatch$ state in which updates the elapsed time in the $display$ every one second (transition $t7$), resets the elapsed time when the button $B$ is pressed (transition $t8$), and returns to the $normal$ state if the button $A$ is pressed (transition $t9$). In addition there are two transitions $t2$ and $t3$ which are executed when buttons $C$ and $D$ are pressed respectively. Since these two transitions are connected from the composite state $on$ to the history state (i.e., $H$), they are executed in both states $noraml$ and $stopnWatch$ and reached to same state as they were before the execution ,e.g., if the button $C$ in the $normal$ state is pressed, the transition $t2$ is executed  and returned to the $normal$ state. 



%Detail information on the execution semantics of statemachine are well addressed in these papers \cite{HAREL1Statechart}. 

==> sections/old-approch.tex <==

\newtheorem{prop}{Proposition}
\newcommand{\RNum}[1]{\uppercase\expandafter{\romannumeral #1\relax}}
\newtheorem{lemma}[theorem]{Lemma}
\section{Methodology} \label{sec:approach}

\subsection{A Conceptual Framework}
Figure \ref{fig:overview} shows a conceptual framework for executing partial models, which consists of three parts (\textit{Static Analysis}, \textit{Automatic Refinement} and \textit{Input-driven Execution}). In the following, we discuss the configuration and the three parts.
\begin{figure*}[t!]
    \centering
    \includegraphics{figures/generic-overview.pdf}
    \caption{A Conceptual Framework for Executing Partial Models}
    \label{fig:overview}
\end{figure*}  
\noindent \textbf{Configuration.} As we discussed in Section~\ref{sec:introduction}, partial model can be executed for different purposes. In all cases, the completeness level of a model is often decided by different stakeholders, based on constraints and goals. We do not have any rule about when a model is complete. Instead, we allow users to specify the completeness level of each component by providing a configuration. Supported levels are $clevels=$\codee{\{complete, partial, absent/ignored\}}. \codee{Complete} components are assumed to be complete, and are not required to be analyzed and refined. \codee{Partial} components are assumed to be incomplete. Thus, their current specification (structure and behavior) is analyzed and refined. \codee{Absent/ignored} components are assumed to have no behavior specification. However, their existence may be necessary for the execution of other (\codee{partial} and \codee{complete}) components, due to the dependency between them. Thus, the \codee{absent/ignored} components are analyzed based on their structure (inputs and outputs) and possible dependencies of other components on them. Then they are given behaviour sufficient for simulation. 
The configuration allows the execution of the models for different purposes. E.g., in the context of the running example which is discussed in Subsection \ref{sec:runningexample}, we can set the \codee{CTR} to \codee{partial}, \codee{SLD} to \codee{complete}, and  \codee{UC} as \codee{absent/ignored} to execute the system for Scenario-1 (evaluation of design decision). For scenario-2 (unit testing), \codee{CTR} should be set to \codee{partial} and the rest of the component as \codee{absent/ignored}. %Note that the appropriate choice of completeness levels is dependent on the purpose and goal of the execution. %E.g., it may be appropriate and useful to label a fully defined component as \codee{absent/ignored}.

%Figure \ref{fig:overview} shows an overview of our approach for executing and debugging the incomplete models of RTE systems, which consists of two phases of \textit{automatic refinement} and \textit{execution}. \\


\noindent \textbf{Static Analysis.} Assuming that the execution semantics of the language is defined, we perform static analysis with respect to the execution semantics to detect the problematic elements that can cause a problem for the execution. Depending on the semantics of the language different types of the problems may be detected. In the context of the state machine, two groups of problems associated with executing partial models: \codee{lack of progress} and \codee{lack of reachability}. The former is related to situations where the execution cannot progress anymore from a certain point. The latter concerns the execution being unable to reach certain defined states. The static analysis is performed on the user-defined model and identifies problematic elements including: (1) missing elements, (2) existing elements with problematic specifications, and (3) missing and un-handled inputs. 

\noindent \textbf{Automatic Refinement.} During the refinement phase, depending on the results of the static analysis and the configuration, the user-defined model is refined automatically using model-to-model transformation techniques. The goal of the refinement is to fix the problematic elements or modify them in such a way that users can provide more information about them during execution. Depending on the modelling languages, certain language constructs can be used to enable models to interact with users during the execution. E.g., for \codee{HSM}s, we use choice-points with certain actions and guards. %Details will be discussed in Subsection \ref{sec:refinment}. 

The refinement should meet the following constraints. (1) Refined models must preserve the original behavior of the user-defined models. (2) The execution of the refined model must not get stuck, assuming proper inputs are provided. (3) The execution of the refined model must be able to reach all defined states in a finite number of execution steps, assuming proper inputs are provided. (4) The execution of the refined model must allow users to select one of the possible options to fix the problematic element. The options must be exhaustive and includes all possible situations which can be applied at design time without limiting the users to only a subset of them. 
%In addition, it is desirable that the refined models be executable using the same method and tool used for the execution of the original models. Thus it is ensured that the refined models can be executed by out-of-box features provided by most MDD tools. Also, the implementation of the framework can be transferred to new tools easily.  

\noindent \textbf{Input-driven Execution.}
The refined model can be executed via interpretation or code generation. During execution, the executed model provides an interface for reading user input either in interactive or batch mode. It is also crucial to provide debugging facilities. Thus, users can investigate the execution before providing inputs.  





\section{Application of the Framework to Partial UML-RT Models}
Generally, the discussed framework can be applied in the context of different modeling languages, to allow execution of partial models. However, since the execution of models is a language-dependent concept, there is no way to provide a generic implementation of the framework using existing techniques and tools. In the rest of this section, we discuss the application of the framework for executing partial UML-RT models. 

\subsection{Static Analysis} \label{sec:staticanalysis}
In the following,  we discuss the details of the static analysis of UML-RT models, with respect to the execution semantic of UML-RT as discussed in Def. ~\ref{sec:semantic}. We categorize the problems based their side effects to lack of progress and reachability. Note that intuitively the lack of progress entails the lake of reachability. \\ %according to their syntax and semantic discussed in Sec.\\ \ref{sec:preliminaries}. 

%This prevents users from testing and debugging of the system. The latter concerns the execution being unable to reach certain defined states.
\subsubsection{{Lack of progress.}} Based on the execution rules of \codee{HSM}s (ref. Def. \ref{def:rules}), the execution of an \codee{HSM} can be stopped due to several issues, which can be divided into two groups, as follows. 

% add rules here
      \textbf{Missing/problematic elements:}  The execution of an \codee{HSM} cannot start, or moves to a stuck configuration, due to the following issues. 
      \begin{itemize} 
      \item \codee{P1}: missing initial state (ref. Def. \ref{def:initconf}), 
      \item \codee{P2}: childless composite states (ref. rule $7$ of  \ref{fig:semantics}), \item \codee{P3}: broken chain  (cf. Rule-$2$ of Fig. \ref{fig:semantics}), 
      \item \codee{P4}: deadlock state  (cf. Rule-$3$ of Fig. \ref{fig:semantics}) , 
      \item \codee{P5}: unexpected messages  (cf. Rule-$5$ of Fig. \ref{fig:semantics}),
      \item \codee{P6} : non-exhaustive guards of choice-points (cf. Rule-$9$ of Fig. \ref{fig:semantics}). 
      \end{itemize}
      Except for P6, the elements with these issues can be queried from the structure of the \codee{HSM}, as follows.  
\begin{align*}
\begin{tabular}{ll}
    \codee{P1} $\leftarrow$ & $\{s_c \in (root(HSM) \cup  \mathcal{S}_c):\; \mathcal{S}_{in} \cap child(s_c) =\emptyset \}$ \\ 
    \codee{P2} $\leftarrow$ & $\{s_c \in (root(HSM) \cup  \mathcal{S}_c):\; child(s_c) =\emptyset \}$ \\ 
    %\codee{R3} & $\{\forall s \in \mathcal{S}_{p} \cup \mathcal{S}_{ch} \cup \mathcal{S}_{in} \cup \mathcal{S}_{jc} \cup \mathcal{S}_{en}: \; \centernot\exists t \in \mathcal{T}, t \in out\_trans(s)\} $ \\
    %\codee{R3} & $\{\forall s \in \mathcal{S}_{p} \cup \mathcal{S}_{ch} \cup \mathcal{S}_{in} \cup \mathcal{S}_{jc} \cup \mathcal{S}_{en}: \; \centernot\exists t \in \mathcal{T}, t \in out\_trans(s)\} $ \\
    \codee{P3} $\leftarrow$ & $\{ s \in \mathcal{S}_{p} \setminus  (\mathcal{S}_{h} \cup \mathcal{S}_{ch}): \;  out\_t(s)=\emptyset\} $ \\
    \codee{P4} $\leftarrow$ & $\{ s \in \mathcal{S}_b: \;   handled(s)=\emptyset \} $ \\ 
    %\codee{P4} $\leftarrow$ & $\{ s \in \mathcal{S}_{c}  : \;  \mathcal{S}_{in} \cap child(s) = %\emptyset \}$ \\
    \codee{P5} $\leftarrow$  & $\{ s \in \mathcal{S}_{b} : \; inp(c) \, \setminus  handled(s) \centernot = \emptyset \} $
\end{tabular}
\end{align*}

As for \codee{P6}, we assume that all choice-points have this problem, (i.e., \codee{P6} $\leftarrow$  $\{ s \in \mathcal{S}_{ch}$\}). This is an overestimation, and covers all possible situations of \codee{P6}. Checking the exhaustiveness of guards of a choice-point during design time is a difficult problem, and requires expensive computation. Thus, fixing this problem at design-time can increase the refinement time significantly, and even make it unsolvable. Also, the applicability of the existing techniques on partial models is not supported by default, and requires extra work and research. 
%The rationale for this assumption will be discussed when we discuss the refinement details. 
\newcommand{\hrulealg}[0]{\vspace{1mm} \hrule \vspace{1mm}}
\begin{algorithm}[t!]
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}
\Input{A UML-RT model \codee{sys} and a configuration \codee{conf} }
\Output{A refined model}
\SetAlFnt{\scriptsize\sf}
\SetKwProg{Fn}{Function}{}{}
\DontPrintSemicolon
{
\hrulealg
Add a debugging interface \codee{dbg\_int} and a debugging agent \codee{dbg\_agent} into \codee{sys} \\
Add ports types with \codee{timing} and \codee{dbg\_int} into \codee{dbg\_agent}
\ForAll(\tcp*[f]{sys.$\mathcal{C}$ (components of sys)}){$c \in$ \codee{sys}.C}{ 
    \Switch(\tcp*[f]{{c.conf} (configuration of c)}){\codee{c.conf}}{ 
        \Case{\codee{partial}}{
            Add port $p$ of type  \codee{dbg\_int} into component $c$ \\
            Add a connection using port $p$ with \codee{dbg\_agent} \\
            $c.\beta \gets$ refineHSM$(c.\beta,\, c)$
        }
        \Case{\codee{absent/ignored}}{
            Add port $p$ of type  \codee{dbg\_int} into component $c$ \\
            Add a connection using port $p$ with \codee{dbg\_agent} \\
            Delete all elements from HSM of $c$ ($c.\beta$) \\
            %$clear(c.\beta)$\\
            $c.\beta \gets$ refineHSM$(c.\beta,\, c)$
        }
        \Other{
            \tcp{No refinement}
        } 
    }
    } 
    \codee{dbg\_agent}$.\beta \gets$ refineHSM$( \codee{dbg\_agent}.\beta,\, c)$
}




\caption{Refinement of a Partial UML-RT Model}\label{refinemodel}
\end{algorithm}

 \textbf{Missing inputs:} A prerequisite for taking an execution step from basic states is the reception of a new message (cf. Rule-4 of Fig. \ref{fig:semantics}) that can enable an outgoing transition from the current state. The execution can be stuck, if the required messages for triggering possible transitions are not produced by the connected components. This can happen for two reasons: (1) the connected component lacks a behavior specification, i.e., components are configured as \codee{absent/ignored}  (\codee{P7}), (2) the behavior of a connected component is partial (\codee{P8}). Detecting \codee{P7} is trivial and can be queried from the interface specification of components. Let ${I}$ be a set of possible input messages of all \codee{partial} and \codee{complete} components, and let ${O}$ be a set of possible outputs messages of \codee{absent/ignored} components, then \codee{P7} $\leftarrow$  ${I}$ $\cap$ ${O}$. \\ 
Detecting \codee{P8} at design time suffers from a similar problem as \codee{P6}. Thus, we overestimate again and assume that all \codee{partial} components have this problem, (i.e., \codee{P8} $\leftarrow$ all \codee{partial} components).  
As we will discuss later, we provide debugging commands for sending messages to the other components from \codee{partial} components, during the execution. That way, users can fix this problem by manually injecting the related messages during the execution. 



\subsubsection{Lack of Reachability.}  Anything causing the lack of progress problem also causes a lack of reachability. There is no way for the execution to reach any state after being stopped. In addition the following Missing/problematic elements can cause a lack of reachability.  
\begin{itemize}
\item \codee{P9}: isolated states refer to states, except for initial and history states, which have no incoming transitions. There is no way for the execution to reach these states.
\item  \codee{P10}: not-takeable transitions originate from a basic or composite state and have no trigger. 
\item 
\codee{P11}: To allow reachability of all states effectively, we define another condition that concerns steering the execution from configurations whose current state is a basic state to any configuration whose current state is any state except composite, choice-point, or initial states. 
Except for \codee{P11}, the elements with these issues can be queried from the structure of a component $c$ with an \codee{HSM} as follows.

\end{itemize}
\begin{align*}
\begin{tabular}{ll}
    \codee{P9} $\leftarrow$ & $\{  s \in \mathcal{S} \setminus (\mathcal{S}_{in} \cup  \mathcal{S}_{h})  : \;  in\_trans(s)=\emptyset \}$ \\ 
    \codee{P10} $\leftarrow$ & $\{  t \in \mathcal{T}: \; src(t) \in \mathcal{S}_{b} \cup \mathcal{S}_{c} \wedge trig(t)= \emptyset \}$ \\ 
    %\codee{R9} $\leftarrow$ & $\{\forall s \in \mathcal{S}_{b} : \; out(c) \, \setminus  handled(s) \centernot = \emptyset \} $ \\
\end{tabular}
\end{align*}

As for \codee{P11}, this capability needs to be addressed in all basic stats, i.e., \codee{P11} $\leftarrow \mathcal{S}_b$.

Note that sets $P1-P11$ are not disjoint and an element may have several issues. For instance, in the context of the running example (ref. Fig. \ref{fig:CTRHSM}), $s_{23}$ is a deadlock state and has a reachability problem, i.e., $S_{23} in P4 \cap P11$ 

\subsection{Refinement of Partial UML-RT Models}
\label{sec:refinment}

%\newcommand{\hrulealg}[0]{\vspace{1mm} \hrule \vspace{1mm}}
%\begin{lstlisting*}
%\centering
%\begin{minipage}{.95\linewidth}
\begin{algorithm*}
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}
\Input{An HSM $sm$ and a component $c$ }
\Output{A refined HSM}
\SetAlFnt{\scriptsize\sf}
\SetKwProg{Fn}{Function}{}{}
\DontPrintSemicolon
{
\hrulealg
\tcp{The following loop refines states in order of their nesting level, with the least deeply nested state (root(HSM)) refined first.}
\ForAll{$s_{c} \in root(sm) \cup ( sm.\mathcal{S} \in  \mathcal{S}_{c})$}{ 
    $dec\_p \gets$ add\_state$(s_{c},\mathcal{S}_{ch})$   \tcp*[f]{Add decision point} 
    
    \uIf(\tcp*[f]{Fix childless composite state (P2)}){$s_{c} \in P2$}{
         $state\_p\_h \gets$ add\_state$(s_{c},\mathcal{S}_{b})$ 
    }
    \uIf(\tcp*[f]{Fix missing initial state (P2)}){$s_{c} \in P1 $}{ 
        add\_state$(s_{c},\mathcal{S}_{in})$ 
    }
    \ForAll{$s_{p} \in (child(s_{c}) \cap P3 \setminus dec\_p$)}{
        add\_trans$(s_p,dec\_p)$ \tcp*[f]{Fix broken chain (P3)}
    }
    \ForAll(\tcp*[f]{Fix non-exhaustive guards for choice-points (P6)}){$s_{ch} \in child(s_{c}) \setminus  dec\_p $}{
        $t_1 \gets$ add\_trans$(s_{ch},dec\_p)$ 
        $t_1.guard \gets \neg \bigvee \big(guard(out\_trans(s_{ch})\big)$ 
    }
    
    \ForAll(\tcp*[f]{Fix unexpected messages (P5), deadlock states (P4), and step 1 of fix for P11}){$s_{b} \in child(s_{c}) \cap P11$}{
        \uIf{$s_{b} \in (P4 \cup P5$)}{
        $t_2 \gets$ add\_trans$(s_{b},dec\_p)$ \\
        $t_2.trig \gets inp(c) \setminus handled(s_{b})$ 
    }
         %$add\_trans(decP,s_{b})$ \tcp*{Fix (R7, 10)}
        %$addTrans(sc,decP,s_{bc})$ \tcp*[l]{Fix isolated states (R7)}
    }
    \ForAll( \tcp*[f]{Fix isolated states (P9) and step 2 of fix for P11}){$s \in (child(s_{c}) \setminus (\mathcal{S}_{in} \cup dec_p) $}{
       $t_3 \gets $add\_trans$(dec\_P,s)$
      % $t_3.guard \gets selection=s$  \tcp{Enable decision making by users}
    }
    
    \ForAll(\tcp*[f]{Fix not-takeable transition (P10)}){$t \in P10$}{
        $t.src=dec\_p$ 
    }
    
    \ForAll (\tcp*[f]{Step 3 of fix for P11}){$s_{cc} \in child(s_{c}) \cap \mathcal{S}_{c}$ }{  
        $ex\_p \gets ex\_p \cup$ add\_state$(s_{cc},\mathcal{S}_{ex})$  \\
        $en\_p \gets en\_p \cup$ add\_state$(s_{cc},\mathcal{S}_{en})$ \\
        $to\_child \gets$ add\_trans$(dec\_p,en\_p \cap child(s_{cc}))$ \\
        $from\_child \gets$ add\_trans$(ex\_p \cap child(s_{cc}) ,dec\_p)$ 
        
    }
    \uIf(\tcp*[f]{Last step of fix for P11} ){$parent(s_{c}) \centernot = \emptyset$}{ %\tcp*[h]{connects sub-states to upper-level } 
        $to\_parent \gets $add\_trans$(dec\_p,ex\_p \cap child(s_{cc}) )$ \\
        $from\_parent \gets$ add\_trans$(en\_p \cap child(s_{cc}),dec\_p)$
    }
    %\uIf{$c =dbgAgent$}{\tcp*[h]{Enable reading commands from external %application}
       % $t_3 \gets addTrans(state\_p\_h,state\_p\_h)$ 
        %$t_3.act \gets send \; \; startTimer$ \\
        %$t_3.trig \gets timeout$
    %}
}

}
\caption{Refinement of \codee{HSM} (refineHSM)}\label{superHSM}
\end{algorithm*}
%\end{minipage}
%\end{lstlisting*}
In the following, we discuss the details of the refinement, applied to fix the problematic elements (\codee{P1-P11}) extracted in the analysis phases. %The refinement is tow-folded. First, structural refinements are applied to prepare infrastructure for the execution, and behavioral refinements are called for \codee{partial} component. Second, behavioral refinement is applied to fix the problematic elements.  


\noindent \textbf{Main Loop of the Refinement.}
Algorithm \ref{refinemodel} shows the main loop of the refinement of a UML-RT model. It takes a UML-RT model and a configuration as inputs. A configuration is a set of tuples $\langle  c \in \mathcal{C}, clevel \in clevels \rangle$, where $c$ is a component and $clevel$ specifies the level of completeness of the component. The algorithm first adds a new component to the model, called \codee{dbg\_agent} with an empty \codee{HSM}, creates a debugging interface, and adds debugging and timing ports into \codee{dbg\_agent}. \codee{dbg\_agent} is responsible for receiving from external applications and transferring \codee{dbg} messages to \codee{partial} and \codee{absent/ignored} components. After setting up \codee{dbg\_agent}, the algorithm tries to apply certain refinements based on the configuration of the components, as follows. 
\begin{enumerate}[leftmargin=*]
    \item For partial components, it adds a debugging port into the components and creates a connection between them and \codee{dbg\_agent}. This allows them to receive the \codee{dbg} message during the execution, which is essential for fixing elements in \codee{P7-P8}. Then it calls the \codee{refineHSM} function, which applies the behavioral refinement to fix the issues (line\# 4-7).
    \item The behavior of absent/ignored components are removed, which results in an empty \codee{HSM}. Then, their empty \codee{HSM} is refined, which results in an \codee{HSM} that can receive and send all possible input and output messages of the component (line\# 8-12).
    \item Finally, the \codee{HSM} of \codee{dbg\_agent} is also refined as a \codee{absent/ignored} component that results in an \codee{HSM} capable of processing debugging commands (line\# 14).

\end{enumerate}

%As shown in \ref{dbgHSM}, it is simple HSM that reacts to incoming messages from other components and processes received debugging periodically. Note, 



\begin{figure*}[ht!]
\centering
\includegraphics[width=16cm,trim={0cm 0cm 6cm 0},clip]{figures/refined-abm-all.pdf}
\caption{Refined \codee{HSM} of AMBController (added elements are coloured blue, and modified elements are coloured red)}
\label{fig:abmrefined}
\end{figure*}

\noindent \textbf{Behavioral Refinement.} Algorithm \ref{superHSM} presents function \codee{refineHSM}, which refines the \codee{HSM} of a component with respect to elements in \codee{P1-P11} except for elements in \codee{P7-P8}. Before discussing the details, let us define $add\_state\,(s_c \in \mathcal{S}_{c}, ty \in \mathcal{S}) \rightarrow \mathcal{S}$ as a function that adds a state of type $ty$ inside the $s_c$ and $add\_trans\,(src, trg \in \mathcal{S}) \rightarrow \mathcal{T}$ as a function that adds a transition from state $src$ to state $trg$. The algorithm iterates over all composite states, and the root of the \codee{HSM}, and refines them in $9$ steps, as follows.
%\vspace{-2mm}
\begin{enumerate}[leftmargin=*]
    \item It creates a choice-point state called \codee{dec\_p}. \codee{dec\_p} is used as a decision point during the execution (line\# 2). When a specification is missing, we refine the \codee{HSM} so that the execution is directed to \codee{dec\_p}. %$state\_p\_h$ is a placeholder for new states that can be defined during the execution by users. {\color{red} More detail on  \codee{dec\_p} and $state\_p\_h$ will be presented in the next Section.}
    \item Fix elements in \codee{P2} which have no child, by adding a new basic state inside the related state (line\# 3-4). Note that the added basic state has issues \codee{P4, P5,} and \codee{P9}, and requires the corresponding fixes.
    \item Fix elements in \codee{P1} which miss initial states, by adding a new initial state inside the related state (line\# 5-6). Note that the added initial state has issue \codee{P3}, and requires the corresponding fixes.
    \item  The elements in \codee{P3} (Broken chain) are fixed by adding a transition from the problematic states to \codee{dec\_p} (line\# 7-8). This ensures that the execution will move to \codee{dec\_p} instead of stopping at the problematic states, and thus users can steer the execution to other states from \codee{dec\_p}. 
    \item Fix elements in \codee{P6} (Non-exhaustive guards) by adding a transition from each choice-point to \codee{dec\_p} so that its guard is set to the negation of the disjunction of the outgoing transitions' guards (line\# 9-10). This ensures that the execution moves to the  \codee{dec\_p} if none of the guards for outgoing transition holds, instead of stopping there. Arguably, this solution is much cheaper than the design time analysis to detect and fix this issue.
    
    \item During this step, a new transition is added from each basic state to \codee{dec\_p} and its trigger is set to all un-handled messages in the state (line\# 12-14). This not only fixes the elements in \codee{P4} (deadlock state) by adding a transition from them to \codee{dec\_p}, but also (1) allows all un-handled messages to be handled as the new transition's trigger (\codee{P5}), and (2) allows the steering of the execution from any basic state to \codee{dec\_p} which is the first step of the fix for elements in \codee{P11}.
    \item A transition is added from \codee{dec\_p} to all basic states and isolated states (line\#15-16). This fixes issue \codee{P9} (isolated states), and also allows the steering of the execution to any basic state from \codee{dec\_p} which is the second part of the fix for \codee{P11}.
    \item To fix non-takeable transitions \codee{(P9)}, their source is changed to \codee{dec\_p} (line\# 17-18). This allows them to be taken whenever the execution reaches \codee{dec\_p}. Since each state has a transition to \codee{dec\_p} which is added in step 6 with a trigger set to all un-handled messages, the non-takable transitions can be activated by any of the un-handled messages. Note that the \codee{dbg} message, which is added using Algorithm~\ref{refinemodel} is assumed to be an un-handled message. 
    \item At the end, an \textit{exit-point} (line\# 20) and an \textit{entry-point} (line\# 21) states are added to each composite state to allow the execution to be steered from their sub-states to states in their parent state and vice-versa, which is the last part of the fix for elements in \codee{P10}. Two transitions \codee{to\_parent} and \codee{from\_parent} allow the execution to be steered from their sub-states to states in their parent state, and transitions \codee{to\_substates} and \codee{from\_upper} allow the execution to be steered from states in their parent state to their sub-states (line\# 19-26).

\end{enumerate}

Note that the refinement algorithms do not contain details for the actions which are added to \codee{HSM}s. E.g., (1) added actions to the \codee{HSM} of \codee{dbg\_agent} for processing and injecting the message \codee{dbg}, (2) guards of outgoing transitions from decision points which are set in a way that allows users to select one of them, (3) actions of incoming transitions to decision points that call a function to read user input. Interested readers can refer to the source code of the refinement \cite{pmdebuggersource}.


\subsubsection{Refinement Result on the Running Example}
%Figure \ref{fig:abmrefined} shows the result of the refinement of the running example for the Scenario-1. Figure \ref{fig:refinedabmstructure} shows the refined structure, in which the \codee{absent/ignored} components have been removed, and their ports have been moved to  \codee{mocking\_agent} and a connection between \codee{mocking\_agent} and \codee{ABMController} is created for sending debugging commands. Figure \ref{dbgHSM} shows the HSM of the \codee{mocking\_agent} which can handle/produce all input/output messages related to \codee{absent/ignored} components. Note that the \codee{mocking\_agent}'s HSM is a refined version of an empty HSM, i.e., the structural model of a component can be executed by receiving the inputs and producing the outputs.

Figure \ref{fig:abmrefined} shows the result of Algorithm \ref{superHSM} on the \codee{ABMController} with \codee{partial} configuration in which transitions and states are annotated with corresponding issues \codee{P1-P11}. Let us review some examples of how the execution can be performed with missing specifications: (1) The transition from \codee{idle} to \codee{showOption} which was not possible in the original model, can be triggered by any of the input messages or \codee{dbg} messages in the refined version to move the execution to state \codee{dec\_p} where users can select one of the outgoing transitions. Note that one of the transitions is $t2$ which was un-takeable in the original model. (2) The execution is stuck in \codee{ch$_{11}$} if a service other than the deposit (\codee{right0} key of the SKB) is selected. In the refined version, the execution moves to \codee{dec\_p} if other services are selected, and users can steer the execution from there.  %Similar situations now are applicable to all other problems. 


%\caption{High-level Grammar of the Debugging Services}
%\label{dbgservices}
%\end{listing}
\subsection{Alternative refinement choices}
Note that the proposed refinement approach are devised experimentally by trying and evaluation of many possible solutions.  We discuss the soundness and correctness of our approach in Section~\ref{}, we show that our approach has a reasonable performance. However, we do not claim that our approach provide the optimal solution of the refinement. For instance, by ignoring some of the problematic cases,  by focusing on fixing certain problems, or by by applying certain assumption there is possibility to refine the models in more efficient way. We leave the optimization of the approach to future work.

\subsection{Execution of Refined Partial UML-RT Models}

In this section, we briefly discuss our method for the execution and debugging of incomplete UML-RT models without dwelling on technical and implementation detail. Interested readers can refer to the project repository \cite{pmdebuggersource}.

As discussed the partial models are refined by adding decision points where elements are missing/partial that allow users to execute the partial models and provide information about the missing/partial element during the execution. This requires a mechanism that (1) enables executed models to obtain user input either in interactive or batch mode, (2) provides debugging features to investigate and modify the execution of the model.%, since deciding about the models without understating the execution and context of the partiality is not useful.   

Figure~\ref{fig:execoverview} shows the execution flow of a refined \codee{HSM} in which a debugging probe is hooked into the execution of an \codee{HSM} by adding relevant actions in the initial transition of the \codee{HSM}. When an \codee{HSM} starts executing, two threads  \codee{main} and \codee{probe} are started but only one of them is active at each time of the execution. Thread $main$ executes the models as specified until it reaches a decision point  where it sends the execution context to the \codee{probe} and waits for the user input. The execution context contains relevant information concerning the execution of the \codee{HSM} such as current state of the execution and a list of possible options to continue the execution. Thread \codee{probe} starts a debugging session (batch or interactive) that allows users to investigate the execution and provide input. At the end of the session, the user input is returned to thread \codee{main} to continue the execution. The interaction between the threads is simply a function call from thread \codee{main} to the \codee{probe} that is implemented using an action in the transitions ending at the decision points. In the following, we review the features that are supported by the debugging probe. 

\label{sec:debuggingprobe}
\lstset{
   language=antlr,
   extendedchars=true,
   basicstyle=\footnotesize\ttfamily,
   showstringspaces=false,
   showspaces=false,
   tabsize=2,
   breaklines=true,
   showtabs=false,
   frame=bt
}
\begin{figure}[t!]
\begin{lstlisting}
grammar ExecRules;
script: execRule+;
execRule: 'rule' rID=ID 'where' '(' where ')' 
when?
    '{' body=scriptStatement*  '}';
when: 'when' '('guard')';
where: State | Component;
statements: scriptStatement | interactiveStatement;
scriptStatement: simpleStatement | complexStatement;
interactiveStatement: (dbgCommands|umlrtCmd) EOF;
umlrtCmd: sendMsgCmd | replyMsgCmd | receipt;
random: 'random';
dbgCommands: viewCmd  | selectCmd| simpleStatement | visited | controlCMD;

\end{lstlisting}
\caption{High-level Grammar of the Debugging Services}
\label{dbgservices}
\end{figure}

\begin{figure}[t!]
    \centering
    \includegraphics{figures/exec-refined-model.pdf}
    \caption{Execution Flow of a Refined \codee{HSM}}
    \label{fig:execoverview}
\end{figure} 


\noindent \textbf{(1) Interactive execution.} If the execution mode is interactive, users are allowed to issue debugging commands listed in \codee{interactiveStatement} of Listing ~\ref{dbgservices}, e.g.,  view and modify variables. Most of debugging services are ported from MDebugger, our previous work on model-level debugging of UML-RT\cite{mojtabadebugging,MDebuggerDemo}. The new debugging commands to facilitate the execution of incomplete models are: (a) \codee{viewCmd} that lists the possible options to continue the execution, (b) \codee{selectCmd} which allows users to select one of the possible options, (c) \codee{simpleStatement} which allows users to define new variables which can be accessed during the debugging session, access all attributes (i.e., \codee{HSM}'s variables and newly defined variables during the debugging session) and modify them using arithmetic expressions, and (d) \codee{umlrtCmd} consists of \codee{send} and \codee{reply} commands which allow users to \codee{send/reply} (inject) messages to other components. In addition, we  support \codee{random} parameter to generate random message payload (only integer) or options depending on the context of the debugging commands.\\ 

\noindent \textbf{(2) Batch execution.}  Interactive execution stops and delays the execution which is not suitable for some situations especially for testing or debugging of time-sensitive systems. For that, a batch execution mode is supported that allows users to provide inputs using a script that consists of execution rules. As shown in \codee{execRule} of Listing ~\ref{dbgservices}, an execution rule consist of a header and a body. The header consists of three parts: rule name, \codee{where}, and \codee{when}. The \codee{where} statement is specified using component and state name and specifies on which elements the rule can be applied. Component/state names can be specified using '*' to cover all components/states. The \codee{when} specifies a guard of the rule. A rule is applied when the current execution context matches the \codee{where} and the \codee{when} is evaluated to true. It is worth mentioning that the execution rules specification method is inspired by the way the transformation rules are specified in rule-based model transformation languages such as ETL~\cite{epsilon2008}. The body of a rule is a sequence of debugging commands which are executed when the rule is applied.

Depending on the current execution context and defined rules, multiple rules may be applicable at each time, but only one rule can be applied at each time. The rule selection is performed according to the following conditions for decision points of an execution context with component $c$ and the current state $s$. 
\begin{enumerate}
    \item Guards of rules whose \codee{where} (i.e., component and state name) is equal to $c$ and $s$  are evaluated based on the order of their appearance in the rules' script file. The first rule whose guard holds is selected and applied.
    \item If (1) is unsuccessful, guards of rules whose state name is exactly equal to $s$ and component name is equal to $*$ or empty are evaluated based on the order of their appearance in the rules' script file. The first rule whose guard holds is selected and applied.
    \item If (2) is unsuccessful, guards of rules whose component name is exactly equal to $c$ and state name is equal to $*$ or empty are evaluated based on the order of their appearance in the rules' script file. The first rule whose guard holds is selected and applied.
    \item If (3) is unsuccessful, guards of rules whose state and component name is $*$ are evaluated based on the order of their appearance in the rules' script file. The first rule whose guard holds is selected and applied.
    \item If none of the above holds, the execution stops and users are asked to provide input to continue the execution. 
\end{enumerate}


Listing \ref{execrulescript} shows a script that includes four samples of the execution rules in the context of the running example.
Let us review some examples of rule selection: (1) For an execution context with component \codee{ABMController} and the current state \codee{idle}, there is no rule that matches both component and state name. Thus \codee{rule1} is selected if \codee{receipt(keyselect)} evaluates to true. Otherwise, \codee{rule3} is selected since it has no guard.
(2) For an execution context with component \codee{PPDMain} and the current state \codee{idle}, there is no rule that matches both component and state name. Two rules (\codee{rule1} and  \codee{rule2}) match the state name. Thus their guards are evaluated in the order of their appearance in the script (i.e., \codee{rule1} and \codee{rule2}).
(3) For an execution context with component \codee{PPDMain} and the current state \codee{readPin} no rule matches the component and the state name. Thus the \codee{rule4} is selected. 

Note that the rule selection process allows definitions of rules that can be applied to more than one execution context. Also, we support \codee{random} generation of users inputs, messages, and messages' payload. These minimize the efforts required to execute partial models, e.g., users can automate the random execution by using \codee{rule-4} that replies to any incoming message randomly and selects one of the possible options to continue execution randomly. 

\lstset{
   language=execRule,
   extendedchars=true,
   basicstyle=\footnotesize\ttfamily,
   showstringspaces=false,
   showspaces=false,
   tabsize=2,
   breaklines=true,
   showtabs=false,
   frame=bt
}  
\begin{figure}[t!]

\begin{lstlisting}
rule rule1 where state idle when  receipt(keyselect) {
    select state  showOption
}
rule rule2 where state idle {
    select state showOption
}
rule rule3 where component ABMController  {
    select state random
}
rule rule4 where component * {
    reply  random
    select state random
}
\end{lstlisting}
\caption{An Example Script of Execution Rules }
\label{execrulescript}
\end{figure}


==> sections/runningexample-backup.tex <==
\subsection{A Running Example}

\label{sec:runningexample}
We use the software system of an Automatic Banking Machine (ABM) system as a running example. 
The top-level structure of the system is shown in Figure \ref{fig:abmstructure} which consists of  eight components: (\codee{AuthorizationGateway (AUTH),}  (\codee{CashDispneser (CDP),} \codee{Display (DSP),} \codee{Printer (PRT),} \codee{CardReader (CDR),} \codee{Pinpad (PPD),} \codee{SelectionKeyboard (SKB),} and \codee{ABMController}. 

Let us assume that a team of two software developers (John, Jenny) is responsible for the development of the ABM system, using an MDE tool and we have the following situation. (1) John is responsible to develop  \textit{ATMController} and \textit{AUTH} and currently is working on the development of \textit{ATMController}. (2) The development of other components (mainly hardware drivers) is assigned to Jenny who is working on the development of \codee{PPD}. %

%\codee{PPD} consists of two components \codee{PPDDriver} and \codee{PPDMain}. The detailed behaviour of \codee{PPDDriver} is not discussed here. Generally, it starts a key-entry session by receiving a \codee{readKeys} message in which users are allowed to enter digits, cancel, confirm, and clear keys. Upon the pressing of the keys, corresponding messages are sent to \codee{PPDMain}, the partial behavior of which is shown in Figure \ref{fig:pinpadmain}. \codee{PPDMain} is supposed to start a pin-entry session, verify the PIN when a confirmation key is pressed, and send back the verification result to \codee{ABMController}. The current version of \codee{PPDMain} behavior misses several elements, such as the handling of the confirm key.% (red part in figure \ref{fig:pinpadmain}) which should lead to pin verification and the sending back of its result.

Figure \ref{fig:atmcontroller} shows the partial behavior of \codee{ABMController}, which plays a key role in our design. It is to control the flow of providing banking services to the users. E.g., a complete flow to withdraw money from an account should start with the help of component \codee{CRD} reading and sending out card data to \codee{ABMController}. Then \codee{ABMController} asks \codee{DSP} to show pages where a user can select \lq withdraw\rq{} from the available services using \codee{SKB}, and enter the amount using \codee{SKB} and \codee{PPD}. Then, \codee{ABMController} passes control to \codee{PPD} to verify the user's pin, upon successful verification of which it sends a withdraw message to  \codee{AUTH}, and finally, upon receiving a response, it performs a proper action, such as dispensing the money and printing a receipt. The state machine in Fig. \ref{fig:atmcontroller} misses several specifications: (a) No detailed behavior is provided for accessing the account balance and other services, e.g., composite state \codee{balance} is empty. (b) It is unclear how execution will progress after reaching state \codee{getAmount}. (c) It is unclear how the transition from state \codee{idle} to \codee{showOptions} can be triggered.  

Let us discuss two exemplary situations where the execution of partial models can be helpful for early debugging and unit testing. 


\textbf{Scenario-1: (Early debugging)} John is an expert in the domain of banking application, but his experience with MDE tools is limited. He wants to execute the current version of the component \codee{ABMController} as shown in~\ref{fig:atmcontroller}, and get early feedback if the flow of the \textit{withdraw} service is correct. Existing MDE tools do not support execution of \codee{ABMController} in the current form, due to two issues: (1) appropriate stubs for all the components need to be created, which is a time-consuming task, (2) even if the stubs are provided, the execution of \codee{ABMController} stops at state \codee{idle} (lack of progress) and then in state \codee{getAmount}, due to the missing specifications, i.e., the trigger of \codee{$t_{12}$} and outgoing transitions from \codee{getAmount} accordingly. Currently, the only possible way to resolve the missing specification is to postpone the debugging until all of them are provided. 


\textbf{Scenario-2: (Unit testing)} Jenny wants to perform unit testing of the current implementations of  \codee{PPDMain}. To do that, all relevant components except \codee{PPDMain} should be replaced by appropriate stubs. Note that even though the design of \codee{PPDDriver} is complete, but it is not reasonable to use that for the unit testing since it requires to be run on hardware which can be time-consuming and complicate the testing process.


==> tables/partialitytypes.tex <==
\begin{singlespace}
\begin{table}[t!]
\begin{threeparttable}
\footnotesize
\caption {Specification of Partiality Types}
\label{tblpartialities}

%\resizebox{\textwidth}{!}{
\tabcolsep=0.2cm
\begin{tabular}[t]{p{0.20cm}p{2.5cm}p{0.0cm}p{3.2cm}}
\hline
 \textbf{Cat.} &\textbf{Type} &\textbf{Specification} \\
 \hline
\hline

 \parbox[c]{2mm}{ \multirow{4}{*} {\rotatebox[origin=c]{90}{$\quad$Explicit$\quad$}}}
 &Not-Executable Transition (EPT)&\multicolumn{2}{p{5cm}}{$\forall t \in \alpha trs(SM*) \bullet (typ(t)=N2x \land tig(t)=\emptyset)$ } 
 %&\multirow{3}{*}{\includegraphics[ trim={5 4 5 3},clip,width= 3 cm, height=1.10cm]{figs/update_time_Sometimes.pdf}}\\ 
 \\ 
 &Not-Visible Transition (EPA)&\multicolumn{2}{p{5cm}}{$\forall t \in \alpha trs(SM) \bullet (act(t)=\emptyset)$} \\
 %\multicolumn{2}{p{10cm}}{\includegraphics[width= 3 cm, height=6mm]{figs/update_time_Sometimes.pdf}}\\ 
 &Dead State (EPD)&\multicolumn{2}{p{5cm}}{$\forall s \in \alpha sts(SM)  \bullet ( typ(s) \in \setminus \{H, F, C\} \land \nexists t \in \alpha trs(SM) \bullet src(t)=s)$} \\
 &Isolate State (EPI)&\multicolumn{2}{p{5cm}}{$\forall s \in S \bullet (\nexists t \in \alpha trs(SM) \bullet (trg(t)=s \land src(t)!=s)$} \\
 &Missing Guard (EPC)&\multicolumn{2}{p{5cm}}{$\forall c \in \alpha sts(SM) \bullet ( typ(c)=Ch \land \nexists t_1,t_2 \in P2x \bullet (src(t_1)=s \land src(t_2)=s \land (grd(t_1)!=\emptyset \lor grd(t2)!=\emptyset))$} \\
\hline
 \parbox[c]{3mm}{ \multirow{4}{*} {\rotatebox[origin=c]{90}{$\quad$ Implicit$\quad$}}}
 &Not-Handled  Input Message (IPUI)&\multicolumn{2}{p{5cm}}{$\forall m \in M_{in} \bullet (\nexists t \in N2x \bullet (trigger(t)=m))$} 
 %&\multirow{3}{*}{\includegraphics[ trim={5 4 5 3},clip,width= 3 cm, height=1.10cm]{figs/update_time_Sometimes.pdf}}\\ 
 \\ 
 &Not-Handled  Input Message (IPUO)&\multicolumn{2}{p{5cm}}{$\forall m \in M_{out} \bullet (\nexists t \in N2x \bullet (send(m) \in action(t)))$} \\
 %\multicolumn{2}{p{10cm}}{\includegraphics[width= 3 cm, height=6mm]{figs/update_time_Sometimes.pdf}}\\ 
 &Full Partiality (IPF)&\multicolumn{2}{p{5cm}}{$(M_{in}!=\emptyset \lor M_{out}!=\emptyset) \land(S=\emptyset) $} \\


\hline
 

\hline


\end{tabular}
\begin{tablenotes}
      \small
      \item  *(The specification is for a given process $\mathcal{P}$ with statemachine $SM(S,s_0,\triangle)$ and input and output messages $M_{in}$ and $M_{out}$ )
\end{tablenotes}

\end{threeparttable}
\end{table}
\end{singlespace}
%%%%%%%%%%%%%
